Accountable Javascript Code Delivery

The internet is a major distribution platform for web applications, but there are no effective transparency and audit mechanisms in place for the web. Due to the ephemeral nature of web applications, a client visiting a website has no guarantee that the code it receives today is the same as yesterday, or the same as other visitors receive. Despite advances in web security, it is thus challenging to audit web applications before they are rendered in the browser. We propose Accountable JS, a browser extension and opt in protocol for accountable delivery of active content on a web page. We prototype our protocol, formally model its security properties with the Tamarin Prover, and evaluate its compatibility and performance impact with case studies including WhatsApp Web, AdSense and Nimiq. Accountability is beginning to be deployed at scale, with Meta's recent announcement of Code Verify available to all 2 billion WhatsApp users, but there has been little formal analysis of such protocols. We formally model Code Verify using the Tamarin Prover and compare its properties to our Accountable JS protocol. We also compare Code Verify's and Accountable JS extension's performance impacts on WhatsApp Web.

==> manifest-manual.tex <==
\subsection{Manifest directives}\label{sec:manifest-manual}

The manifest file should contain the list of all active contents 
in the same order they appear in the Html document of the web page. 
% TODO mention the difference between CSP in terms of order.
The file is in a JSON tree format.
The manifest file may contain the following directives in the top level
that gives general information about the web page, transparency logs and the developer:
%TODO talk about the dynamic-static distinction. somewhere?

\begin{itemize}[leftmargin=1.2em]
	\item "$\manname$" : name of the manifest file (optional).
	\item "$\manmanversion$" : version number of the manifest file (required).
	\item "$\mandescription$" : short description of the manifest file (optional).
	\item "$\textURL$" : the URL of the website (required).
	\item "$\mancontents$" : the list of the active contents are under this key.
	
\end{itemize}

The following keys can be used in the second level (under contents key): some of the keys may be required depending on the type of the active content. 

\begin{itemize}[leftmargin=1.2em]
	\item "$\manseq$" : the sequence number of the content (optional if the content is $\dynamic$).

	\item "$\manname$" : name of the content (optional).

	\item "$\manversion$" : version number of the content (optional).

	\item "$\mantype$" : the type of the content. It can be "$\inline$", "$\eventhandler$", "$\external$" or "$\iframe$". The $\mantype$ is required for each manifest section.

	\item "$\mantrust$" : the trust setting of the content declaration. It can be "$\assert$", "$\blindtrust$", "$\delegate$". The trust setting is required for the $\external$ and $\iframe$ types.

	\item "$\mansrctype$" : iframe resource type. The value can be "$\external$", "$\script$" or "$\mansrcdoc$". It is optional and default value is "$\external$". If the value is "$\external$" then $\mansrc$ directive's value must be a $\URL$, whereas for "$\script$" or "$\mansrcdoc$",
	a $\manhash$ value must be given in $\mansrc$ attribute.

	\item "$\mansrc$" : If the $\mantype$ is "$\external$" or "$\iframe$" then it is also required. 
	For $\external$ a $\textURL$ is expected. For $\iframe$ the value depends on the $\mansrctype$ 
	as stated above. It's also required if the content is blindly trusted by the developer and a $\textURL$ is always expected in this case.
	%
	% \item "$\mansrctype$" : iframe resource type. The value can be "$\external$", "$\script$" or "$\mansrcdoc$". It is optional and default value is "$\mansrc$". 
	% %TODO there was a manlist here, should be added later
	% \item "$\mansrc$" : iframe source (required for iframes). The value depends on the $\mansrctype$. It can be a URL for "$\manlink$", a hash value for "$\script$" and "$\mansrcdoc$". \comment{What's the difference to the $\manlink$ attribute if $\mansrctype$ is $\manlink$. Also, it is a bit confusing that $\manlink$ is both a key on its own and a value for $\mansrctype$.}
	% %\comment{a list of possible URLs for "$\manlist$"}. 
	% By default a URL is expected if "$\mansrctype$" is not given.
	\item "$\mansandbox$" : Required if the content is iframe and the trust is "$\blindtrust$".

	\item "$\manhash$" : if the trust is set for assert (or not given), the cryptographic hash is required. Supported hash algorithms are sha256, 384 and 512. The format is the prefix that shows the hash algorithm followed by a dash e.g. "sha256-" and base-64 encoded hash of the resource.
	% That is the name of the hash method followed by a dash and followed by a base64 on the hash result.
	\item "$\mancrossorigin$" : the CORS setting attribute. If the content is external, this is required. 
	\item "$\dynamic$" : indicates  whether element is part of the initial DOM or dynamically added after the Window load event.  Optional with default value `false'.
	% We changed this functionality, update it
	\item "$\manload$" : indicates if the script is loaded synchronously or asynchronously. The value can be "$\sync$", "$\async$" or "$\defer$". It is optional and the default value is "$\sync$".
\end{itemize}

% An example of manifest.json file is available in ~\cite{manifestlink}.

% \begin{itemize}[leftmargin=1.2em]
% 	\item The files are under "order" section.
% 	\item "seq" : means the sequence number (optional)
% 	\item "name" : the name of \ac{JS} library (optional)
% 	\item "version" : the version of \ac{JS} library (required if the library is external)
% 	\item "type" : There are four types of \ac{JS} library "external", "inline", "local" and "event_handler" (required)
% 	\item "link" : The URL of external library (required if the library is external)
% 	\item "SRI" : The SRI value of the library (required if the library is external)
% 	\item "crossorigin" : The crossorigin value of external library (required if the library is external)
% 	\item "script" : Used for inline \ac{JS} or event handlers. The hash (SHA-256, 384 or 512) of entire inline script or entire tag including event handler must be written under this tag (required for type inline and event_handler)
% 	\item "src" : Used for local \ac{JS} file. SRI is not used for local \ac{JS}. But we can still use it. Browser fetches the \ac{JS} file in $<script>$ tags from the server during parsing. 
% \end{itemize}

\subsubsection{Details on hash computation}

\begin{itemize}[leftmargin=1.2em]
    \item $\mansrcdoc$ : The HTML document of the $\iframe$ can be written in
                            $\mansrcdoc$ attribute and it overrides the $\mansrc$ attribute (if used).
                            %
                            %TODO src_doc missing reference
                            %
                            This type of iframe also cannot be declared with the $\delegate$ value 
                            and the $\assert$ method can be applied 
                            as the previous type $\script$, 
                            except in the first operation the $\manhash$ 
                            should be computed on $\mansrcdoc$ value and $\mansrc$ should be ignored.
                            \comment{I didn't get this sentence.}

                        The first operation is to compute
                        % 
                        the $\manhash$ on the $\mansrc$ attribute and assign it 
                        to the $\manhash$ attribute of the manifest block. 
                        % excluding the HTML document.
                        The second operation is about providing assurance 
                        for the HTML document inside the $\iframe$.
                            %
                            This can either be achieved by computing the $\manhash$ on the $\iframe$ 
                                element's $\outerhtml$ property~\cite{Dom-outerHtml}
                                and assigning it to the $\manmanifest$ attribute of the manifest block
                                %TODO// maybe manifest is not a good name here
                                or by providing a list of manifest blocks 
                                for the active elements inside the \iframe's HTML document and place 
                                    this list under the $\manmanifest$ attribute.
                                    %
                                    The other directives, that are also used in common with other elements 
                                    or specific to $\iframe$ (e.g., $\mansandbox$), 
                                        are intuitive and specified in Section~\ref{sec:manifest-manual}.
\end{itemize}

\subsection{Manifest delivery}

For obtaining the manifest as quickly as possible,
the prototype is designed to give priority to take 
the manifest from the response header directly.
%
If the manifest is available in the response headers, 
the other directives for obtaining the manifest will be ignored,
otherwise
the $\accjsheader$ is searched in response headers and meta-tags.

